Non-isotopic surfaces in $T^4\#(S^2\times S^2)$: an example

We prove that there exist infinitely many embedded tori with a common geometric dual in $T^4\#(S^2\times S^2)$ that are homotopic, diffeomorphic, but not isotopic to each other, even after arbitrary many external stabilizations. These surfaces are obtained by applying the Norman trick to a fixed immersed surface, using non-homotopic tubing arcs. The isotopy classes of these surfaces are distinguished by homotopy classes of the 2-handles (relative to the boundary) in the complement of the image of the $0$- and $1$-handles.

==> Construction_backup_.tex <==
%!TEX root = main.tex

Pick a basepoint $x_0$ on $T^2$ and fix a handle decomposition $H_0\cup H_1\cup H_2$ on $T^2$, where $H_0$ is the single 0-handle containing $x_0$, $H_1=H_1^1\cup H_1^2$ is the union of two 1-handles and $H_2$ is the 2-handle. Let $e_0\cup e^1_1\cup e^2_1\cup e_2$ be the corresponding cell structure on $T^2$. We require that $e_0=x_0$.

Let $X=T^4\#(S^2\times S^2)$, where we require the connected sum takes place in the disks $D_1\times D_2\subset T^2\times T^2=T^4$ and $D_1\times D_2\subset S^2\times S^2$, where $D_1,D_2$ are disks. Fix points $b_1\in T^2-D_2$ 
 and $q\in  S^2-D_2$, then there is a standard inclusion:
\begin{equation}\label{eq: ib1}
    i_{b_1}:T^2\rightarrow T^2\times T^2-(D_1\times D_2)=T^4-D^4, \quad x\mapsto (x,b_1).
\end{equation}

\begin{figure}
	\begin{overpic}[width=0.2\textwidth]{./figures/trivial path}
        \put(-15,32){$T^2$}
        \put(45,72){$b_1$}
        \put(35,43){$b_2$}
        \put(47,12){$\partial D_2$}
        \put(43,56){$\overline{\gamma}_0$}
	\end{overpic}
	\caption{Trivial path $\overline{\gamma}_0$}
    \label{fig:trivial path}
\end{figure} 
Pick another $b_1^{\prime}\in D_1, b_2\in \partial D_2$ and construct a path $\gamma_0$ in $T^4-D^4$ from $i_{b_1}(T^2)$ to $\partial D^4$ as follow: we first pick a trivial path $\overline{\gamma}_0:[0,1]\rightarrow T^2-\operatorname{int}D_2$ shown as in Figure \ref{fig:trivial path}, then define $\gamma_0(t)=(b_1^{\prime},\overline{\gamma}_0(t))$. Similarly, we can construct a trivial path $\gamma_1$ in $S^2\times S^2-D^4$ with $\gamma_1(0)=\gamma_0(1),\gamma_1(1)\in S^2\times\{q\}$. Then we can form the tubed surface $\Sigma_0=(T^2\times\{b_1\})\#_{\gamma_0\cdot\gamma_1}(S^2\times\{q\})$. Let $i_0:T^2\rightarrow \Sigma_0$ be a diffeomorphism obtained by modifying $i_{b_1}$ near $(b_1^{\prime},b_1)$. The map $T^2\hookrightarrow X$ obtained by composing $i_0$ with the inclusion $\Sigma_0\hookrightarrow X$ will be still denoted by $i_0$ by abuse of notation. Obviously, $\Sigma_0$ has a geometric dual $G=\{p\}\times S^2$, where $p\in S^2-D_1$.

For any $\sigma\in\pi_1(\Sigma_0)$, we construct another embedding $i_{\sigma}: T^2\rightarrow X$ as follow:

Pick a small disk $B_1\subset S^2$ such that $p\in\partial B_1$. Let $p_1, p_2$ be two distinct points in $\partial B_1\setminus\{p\}$, $G_i=\{p_i\}\times S^2$, $i=1,2$ and $\gamma_{\sigma}: I\rightarrow \Sigma_0$ be an embedded path with $\gamma_{\sigma}(0)=y_1=(p_1,q),\gamma_{\sigma}(1)=y_2=(p_2,q)\in (S^2\times S^2)-(D_1\times D_2)\subset X$. Since $B_1$ is contractible, $\gamma_{\sigma}$ can be viewed as an element in $\pi_1(\Sigma_0)$. We require $\gamma_{\sigma}$ to represent the given $\sigma\in\pi_1(\Sigma_0)$. Form the tubed sphere $G_{12}=G_1\#_{\sigma}\overline{G_2}$. Here, $\overline{G_2}$ denotes the sphere with reversal orientation. 

Let $\kappa:I\rightarrow X$ be another embedded path from $\Sigma_0$ to $G_{12}$ with $\operatorname{int} \kappa \cap (\Sigma_0\cup G_{12})=\emptyset$, and $\operatorname{im}\kappa$ lying very close to $S^2\times\{q\}$, see Figure \ref{fig:Sigma_1}. More precisely,
$S^2\times S^2$ has local model $B_1\times B_2$, where $B_2$ is a small disk in $S^2$ such that $q\in \operatorname{int}B_2$. Pick $\widetilde{p}\in\operatorname{int}B_1, \widetilde{q}\in\operatorname{int}B_2-\{q\}$, such that $(\widetilde{p},q),(p_1,\widetilde{q})\notin G_{12}$. Let $\kappa$ be the straight line in $B_1\times B_2$ from $(\widetilde{p},q)$ to $(p_1,\widetilde{q})$. We may perturb $\kappa$ slightly in order to avoid intersecting with $G_{12}$. Denote the tubed surface $\Sigma_0\#_{\kappa}G_{12}$ by $\Sigma_{\sigma}$. Let $i_{\sigma}:T^2\rightarrow \Sigma_{\sigma}$ be a diffeomorphism obtained by modifying $i_0$ near $\kappa(0)\in\Sigma_0$. As before, we also view $i_{\sigma}$ as an embedding of $T^2$ in $X$. 

After tubing, $G_{12}$ does not intersect with $\Sigma_0$. Therefore $G$ intersects $\Sigma_{\sigma}$ at $(p,q)\in X$ transversely, thus is also a geometric dual of $\Sigma_{\sigma}$.  We require that  $i_0|_{H_0\cup H_1}=i_{\sigma}|_{H_0\cup H_1}$.
\begin{figure}
	\begin{overpic}[width=0.6\textwidth]{./figures/Construction of sigma_1}
        \put(-9,45){$\Sigma_0$}
		\put(200,23){$G$}
		\put(215,40){$\{p_2\}\times S^2$}
		\put(214,56){$\{p_1\}\times S^2$}
        \put(15,33){$\sigma$}
        \put(198,55){$\kappa$}
	\end{overpic}
	\caption{The construction of $\Sigma_{\sigma}$}
    \label{fig:Sigma_1}
\end{figure}

Let $X^{\prime}$ be the closure of $X-\nu(i_0(H_0\cup H_1))$ in $X$, where $\nu(H_0\cup H_1)$ is a regular neighborhood of $i_0(\nu(H_0\cup H_1))$ in $X$. Let $D^2_0, D^2_{\sigma}$ be the intersections $\Sigma_0\cap X^{\prime}, \Sigma_{\sigma}\cap X^{\prime}$, respectively. Then $D^2_0, D^2_{\sigma}$ are two properly embedded disks in $X^{\prime}$, which coincide with each other on the boundary.




